Can Prompt Modifiers Control Bias? A Comparative Analysis of Text-to-Image Generative Models

It has been shown that many generative models inherit and amplify societal biases. To date, there is no uniform/systematic agreed standard to control/adjust for these biases. This study examines the presence and manipulation of societal biases in leading text-to-image models: Stable Diffusion, DALL-E 3, and Adobe Firefly. Through a comprehensive analysis combining base prompts with modifiers and their sequencing, we uncover the nuanced ways these AI technologies encode biases across gender, race, geography, and region/culture. Our findings reveal the challenges and potential of prompt engineering in controlling biases, highlighting the critical need for ethical AI development promoting diversity and inclusivity. This work advances AI ethics by not only revealing the nuanced dynamics of bias in text-to-image generation models but also by offering a novel framework for future research in controlling bias. Our contributions-panning comparative analyses, the strategic use of prompt modifiers, the exploration of prompt sequencing effects, and the introduction of a bias sensitivity taxonomy-lay the groundwork for the development of common metrics and standard analyses for evaluating whether and how future AI models exhibit and respond to requests to adjust for inherent biases.

==> sec/2_Motivation.tex <==
\section{Motivation} 
\label{sec:Motivation}
% The burgeoning field of text-to-image generation models, exemplified by technologies has introduced groundbreaking capabilities in visual content creation. These models, powered by vast datasets and advanced algorithms, promise a new era of creativity and efficiency. However, with great power comes great responsibility, particularly in ensuring that these innovations do not perpetuate or amplify societal biases.

%  Our motivation for this study arises from preliminary observations indicating significant disparities in how these models represent concepts with inherent cultural and geographic origins, such as "monk," a figure predominantly associated with Asian cultures and historically male roles.

% Initial distributions of generated images for a generic "monk" prompt across different models revealed a pronounced bias towards depicting monks as Asian males. While such a bias might reflect historical and geographical realities, the extent of its representation raises questions about the underlying datasets and algorithmic processes guiding these models which is present in Tab.~\ref{tab:Monk}. Notably, Firefly demonstrated a more balanced distribution across genders and racial backgrounds, suggesting a divergent approach to handling or mitigating biases. 


Our investigation into the realm of text-to-image generation models is driven by initial observations that highlight a significant variance in the depiction of culturally and geographically nuanced concepts, such as the archetype of the "monk," traditionally associated with Asian cultures and male roles. The preliminary analysis of image outputs for a generic "monk" prompt across various models unveiled a marked inclination towards representing monks as Asian males, as detailed in Tab.~\ref{tab:Monk}. This tendency, while possibly reflective of historical accuracies, prompts scrutiny over the data and algorithms that inform these models, particularly in how they navigate cultural and gender biases. Interestingly, the Firefly(FF) model showcased a notably more balanced gender and racial representation, indicating a unique approach to bias attenuation.

\begin{table}[ht]
\centering
\footnotesize
% \scriptsize

\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Model} & \textbf{Male / Female} & \textbf{Asian / Others} & \textbf{Total Samples} \\
\hline
SD & 50 / 0 & 50 / 0 & 50 \\
DallE & 36 / 0 & 35 / 1 & 36 \\
FF & 28 / 24 & 5 / 47 & 52 \\
\hline
\end{tabular}
\caption{Distribution of Gender and Race for "Monk" Prompt}
\label{tab:Monk}
\end{table}


% This observation becomes even more intriguing when we consider compound prompts designed to challenge the models with non-traditional representations, such as a "Monk who is black." As results shown in Tab.~\ref{tab:MonkBlack}, it is crucial to note that despite the specific prompt for a "monk who is black," Stable Diffusion and Dall$\cdot$E predominantly continued to produce images reflecting the Asian cultural background, underscoring the models' tendency to prioritize historical and cultural associations over the explicit instructions in the prompt.
The complexity of this issue deepens when examining the models' responses to compound prompts aimed at eliciting non-traditional representations, such as a "Monk who is black," shown in Tab.~\ref{tab:MonkBlack}. Notably, despite explicit instructions, Stable Diffusion(SD) and Dall$\cdot$E 3(DallE/DE) predominantly produced imagery tied to Asian cultural markers, highlighting a proclivity to default to historical and cultural stereotypes over direct prompt cues.


\begin{table}[ht]
\centering
% \scriptsize
\footnotesize
\caption{Distribution of Race for "Monk Who is Black" Prompt}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Model} & \textbf{Asian} & \textbf{Black} & \textbf{Others} & \textbf{Total Samples} \\
\hline
SD & 50 & 0 & 0 & 50 \\
DallE & 35 & 3 & 15 & 53 \\
FF & 14 & 26 & 12 & 52 \\
\hline
\end{tabular}
\label{tab:MonkBlack}
\end{table}

% The stark differences in how each model responded to these prompts, especially with Firefly's unexpected shift towards a more egalitarian distribution, underscore the complexity of bias within AI systems. These discrepancies not only highlight the potential for inherent biases to influence content generation but also raise critical questions about the models' adherence to real-world demographics and cultural sensitivities. Is the goal of these models to mirror historical and statistical realities, or should they strive for an idealized representation that champions diversity and equality? Furthermore, Firefly's approach, while commendable for its inclusivity, prompts a debate on the accuracy and appropriateness of overly equalized distributions that may not align with actual demographics.
The divergent responses to these prompts, particularly Firefly's shift towards equitable representation, spotlight the nuanced challenge of bias within AI systems. Such variance raises pivotal questions about the objective of these models in reflecting the diversity of human experience. Should they aim to accurately mirror historical and sociodemographic realities, or aspire towards an idealized inclusivity that may diverge from factual representation? While Firefly's inclusive approach is laudable, it ignites debate on the validity of achieving balance at the potential expense of demographic authenticity.


% This study is motivated by the need to delve deeper into these questions, aiming to unpack the layers of bias embedded within text-to-image generation models. By comparing the response of these models to both single(standard) and compound prompts, we seek to illuminate the mechanisms of bias formation and propagation in AI-driven content creation. Our goal is not only to identify and quantify biases but also to explore methodologies for their mitigation, thereby contributing to the development of more fair, equitable, and culturally sensitive AI technologies.

% This adjustment emphasizes the influence of cultural background and historical context on the generated images, especially in contrast to the explicit instructions provided in the prompts, setting the stage for a deeper investigation into bias mitigation and the fidelity of AI models to diverse inputs.

Motivated by these observations, our study aims to dissect and understand the bias embedded within these AI technologies. By evaluating the models' outputs against both standard and modified prompts, we intend to shed light on the origins and impacts of bias in AI-generated imagery. Our objective extends beyond merely identifying bias to exploring avenues for its rectification, with the ultimate goal of fostering the development of AI tools that are both fair and culturally attuned. Through this endeavor, we hope to contribute to the broader discourse on ethical AI development, particularly in the context of generating visual content that respects and reflects the rich tapestry of human diversity.

\vspace{-5pt}

